Decoding Time Series with LLMs: A Multi-Agent Framework for Cross-Domain Annotation

Time series data is ubiquitous across various domains, including manufacturing, finance, and healthcare. High-quality annotations are essential for effectively understanding time series and facilitating downstream tasks; however, obtaining such annotations is challenging, particularly in mission-critical domains. In this paper, we propose TESSA, a multi-agent system designed to automatically generate both general and domain-specific annotations for time series data. TESSA introduces two agents: a general annotation agent and a domain-specific annotation agent. The general agent captures common patterns and knowledge across multiple source domains, leveraging both time-series-wise and text-wise features to generate general annotations. Meanwhile, the domain-specific agent utilizes limited annotations from the target domain to learn domain-specific terminology and generate targeted annotations. Extensive experiments on multiple synthetic and real-world datasets demonstrate that TESSA effectively generates high-quality annotations, outperforming existing methods.

==> 2_preliminary.tex <==
%\section{Preliminary and Problem Statement}
%\subsection{Notations}
%\suhang{use text to define few notations, e.g., time-series and annotation, move the table to appendix} \minhua{I will delete the subsection, and mention that more details of the notation will be in Appendix~\ref{appendix:notations}.}

\nop{
\subsection{Time Series Annotation}
% \noindent \textbf{Time Series Annotation}
% Given a time series $\{\mathbf{x}_i\}_{i=1}^{L}=(\mathbf{x}_1,\cdots,\mathbf{x}_L)$, where $L$ is the number of past timestamps and $\mathbf{x}_i=(\mathbf{x}_{1i},\cdots,\mathbf{x}_{mi})^{T}\in\mathbb{R}^C$ represents the data from $C$ different channels at timestamp $i$, the objective of time series annotation is to generate a descriptive general annotation $e_g$ or domain-specific annotation $e_s$.

% the objective of time series annotation is to generate a descriptive annotation or interpretation that captures important patterns, trends, or features in the time series. 
% For simplicity, in this paper, we focus on the univariate time series $\mathbf{x}=(x_1,\cdots,x_L)$, where each $x_i\in\mathbb{R}, \forall i\in L$. And it is easy to extend our method to multivariate time series data. \suhang{If you are doing experiments on multivariate time series, then do not say focus on univariate time series, just describe from multivariate TS perspective}

Time series annotation refers to the process of interpreting time series data by providing meaningful context or insights that highlight important patterns, events, or anomalies within the data. These annotations aim to make complex temporal information more understandable, especially in multivariate time series where multiple variables interact over time. There are two types of annotations, general annotations and domain-specific annotations, are involved. Specifically, general annotations are domain-agnostic and highlight patterns that are universally significant, regardless of the specific domains, which are useful for generic analysis and can serve as a baseline for further domain-specific investigations. They focus on common patterns and insights that are relevant across multiple domains.  Domains-specific annotations are tailored to a particular domain and leverage specialized knowledge to identify patterns meaningful only within that context. They incorporate specialized terminology and insights that require domain expertise to interpret accurately, which benefits domain-specific downstream tasks, such as clinical decision-making in healthcare or fault detection in engineering systems.}

% By offering explanations that contextualize the data—either in general terms or using domain-specific terminology—time series annotations facilitate accurate analysis, forecasting, and decision-making across various fields such as manufacturing, finance, and healthcare.

% Note that this involves two types of annotations, general annotation $e_g$ and domain-specific annotation $e_s$. Specifically, $e_g$ is domain-agnostic. It highlights patterns that are universally significant, regardless of the specific field. These annotations are useful for generic analysis and can serve as a baseline for further domain-specific investigation. $e_s$ is tailored to a particular domain. It leverages specialized knowledge to identify patterns that are meaningful only within that context, which are critical for domain-specific downstream tasks, such as clinical decision-making in healthcare or fault detection in engineering systems. 
% \suhang{I do not think this paragraph should appear here. You are defining the problem, i.e., what are given and what's your output. The general annotation is part of your approach for tackling the problem}


% a general annotation $e_g$ and a domain-specific annotation $e_s$.

% This may include identifying key characteristics such as seasonality, trend, anomalies, correlation between channels, and other relevant temporal dynamics. The generated annotation should provide insights that are both comprehensive and interpretable, enabling users to understand the underlying structure of the time series.

\nop{
\subsection{Limitations of Baselines}
One natural solution to solve this problem is to directly apply LLMs to interpret time series data. However, LLMs tend to capture only simple patterns and often produce inaccurate annotations. For instance, Figure~\ref{} presents an annotation generated by applying GPT-4o to interpret the original univariate time series data in Figure~\ref{}. The model focuses solely on identifying the trend, missing other important patterns. Furthermore, these annotations often contain hallucinations, further complicating their interpretation for users.
}

% When extended to multivariate time series data, as shown in Figure~\ref{}, LLMs annotate each variable independently, disregarding the relationships between variables. \suhang{you criticise existing work annotate each variable independently, then reviewer would expect you to solve this issue. Either delete this point or give details on how you solve this issue in the methodology part} Furthermore, these annotations often contain hallucinations, further complicating their interpretation for users.

% \suhang{Formally define the Cross-Domain Multivariate Problem you are studying}
\nop{\subsection{Problem Statement}
\noindent\textbf{Cross-Domain Time Series Annotation}.
Given several source domains $\{\mathcal{D}_{s_1},\mathcal{D}_{s_2},\ldots\}$ and a target domain $\mathcal{D}_t$, where $\{{e}^1_{s_i},{e}^2_{s_i},\ldots\}$ are the domain-specific annotations~\footnote{We do not require the quality and source of domain-specific annotations.} from the source domain $\mathcal{D}_{s_1}$ and $\{{e}^1_{t},{e}^2_{t},\ldots\}$ are the limited domain-specific annotations from target domain $\mathcal{D}_t$, respectively. 
Suppose $\mathbf{X}=(\mathbf{x}_1,\cdots,\mathbf{x}_L)$ is a time series in $\mathcal{D}_t$, where $L$ is the number of past timestamps and $\mathbf{x}_i=({x}_{1i},\cdots,{x}_{Ci})^{T}\in\mathbb{R}^C$ represents the data from $C$ different channels at timestamp $i$. The objective of cross-domain time series annotation is to generate the general annotation $e_g$ and domain-specific annotation $e_s$ for $\mathbf{X}$ based on the annotations from the source domains and the target domain, respectively. More details of the notations are in Appendix~\ref{appendix:notations}.}
% generate a descriptive general annotation $e_g$ or domain-specific annotation $e_s$.


